An Independent Analysis of the Six Recently Claimed Exomoon Candidates

It has been recently claimed that KOIs-268.01, 303.01, 1888.01, 1925.01, 2728.01 & 3320.01 are exomoon candidates, based on an analysis of their transit timing. Here, we perform an independent investigation, which is framed in terms of three questions: 1) Are there significant excess TTVs? 2) Is there a significant periodic TTV? 3) Is there evidence for a non-zero moon mass? We applied rigorous statistical methods to these questions alongside a re-analysis of the Kepler photometry and find that none of the KOIs satisfy these three tests. Specifically, KOIs-268.01 & 3220.01 pass none of the tests and KOIs-303.01, 1888.01 & 1925.01 pass a single test each. Only KOI-2728.01 satisfies two, but fails the cross-validation test for predictions. Further, detailed photodynamical modeling reveals that KOI-2728.01 favours a negative radius moon (as does KOI-268.01). We also note that we find a significant photoeccentric for KOI-1925.01 indicating an eccentric orbit of e>(0.62+/-0.06). For comparison, we applied the same tests to Kepler-1625b, which reveals that 1) and 3) are passed, but 2) cannot be checked with the cross-validation method used here, due to the limited number of available epochs. In conclusion, we find no compelling evidence for exomoons amongst the six KOIs. Despite this, we're able to derive exomoon mass upper limits versus semi-major axis, with KOI-3220.01 leading to particularly impressive constraints of Ms/Mp < 0.4% [2 sigma] at a similar relative semi-major to that of the Earth-Moon.

==> planettable.tex <==
\begin{table*}
\caption{
All summary statistics reported represents the median and surrouding
1\,$\sigma$ credible interval, with the exception of $e_{\mathrm{min}}$
for which we report the mode and 1\,$\sigma$ interval.
Error for $P$ is omitted for brevity, but are quoted to the same number
of decimal places as found when rounding the uncertainty to 2 s.f.
* solution presented a second mode at grazing configuration that was
rejected.
\dagger assumed circular due to multiplanetary configuration
\ddagger TTV fit favored
} % title of Table
\centering % used for centering table
\begin{tabular}{c c c c c c c c} % centered columns (8 columns)
\hline\hline %inserts double horizontal lines
KOI &
$P$\,[d] & 
$R_P/R_{\star}$ &
$b$ &
$a/R_{\star}$ &
$e_{\mathrm{min}}$ &
$R_P$\,[$R_{\oplus}$] &
$S_{\mathrm{circ}}$\,[$S_{\oplus}$] \\ [0.5ex] % inserts table
%heading
\hline % inserts single horizontal line
701.04	& 267.2878 & $0.02046_{-0.00080}^{+0.00067}$ & $0.0527_{-0.064}^{+0.048}$ & $233.0_{-4.7}^{+4.9}$ (\dagger) & 0 (\dagger) & $1.499_{-0.066}^{+0.060}$ & $0.456_{-0.027}^{+0.030}$ \\
3138.02	& 
4742.01*& 112.3053 & $0.0213_{-0.0018}^{+0.0031}$ & $0.49_{-0.33}^{+0.34}$ & $126_{-41}^{+22}$ & $0_{-0}^{+0.22}$ & $1.46_{-0.13}^{+0.22}$ & $1.00_{-0.28}^{+1.24}$ \\
5387.01*& 297.819 & $0.0150_{-0.0016}^{+0.0019}$ & $0.47_{-0.32}^{+0.34}$ & $130_{-464}^{+35}$ & $0.60_{-0.17}^{+0.21}$ & $1.03_{-0.11}^{+0.14}$ & $0.84_{-0.32}^{+1.17}$ \\
5870.01*& 132.12 & $0.0102_{-0.0061}^{+0.0033}$ & $0.52_{-0.35}^{+0.33}$ & $270_{-200}^{+250}$ & $0.70_{-0.40}^{+0.21}$ & $0.67_{-0.40}^{+0.23}$ & $0.22_{-0.16}^{+2.97}$ \\
5971.01*& 493.315 & $0.0166_{-0.0018}^{+0.0023}$ & $0.46_{-0.32}^{+0.35}$ & $790_{-250}^{+240}$ & $0.73_{-0.23}^{+0.10}$ & $1.44_{-0.16}^{+0.20}$ & $0.041_{-0.017}^{+0.048}$ \\
8174.01*\ddagger	& 295.030 & $0.00852_{-0.00068}^{+0.00090}$ & $0.47_{-0.32}^{+0.30}$ & $130_{-35}^{+23}$ & $0.43_{-0.15}^{+0.22}$ & $0.816_{-0.073}^{+0.093}$ & $2.29_{-0.65}^{+2.00}$ \\
%\hline
%719.03	& 
%2124.01	& 
%2173.02	& 
%3284.01	& 
\hline\hline %inserts single line
\end{tabular}
\label{tab} % is used to refer this table in the text
\end{table*}
